Isospin Breaking Effects on the Lattice

Isospin symmetry is not exact and the corrections to the isosymmetric limit are, in general, at the percent level. For gold plated quantities, such as pseudoscalar meson masses or the kaon leptonic and semileptonic decay rates, these effects are of the same order of magnitude of the errors quoted in nowadays lattice calculations and cannot be neglected any longer. In this talk I discuss the methods that have been developed in the last few years to calculate isospin breaking corrections by starting from first principles lattice simulations. In particular, I discuss how to perform a combined QCD+QED lattice simulation and a renormalization prescription to be used in order to separate QCD from QED isospin breaking effects. A brief review of recent lattice results of isospin breaking effects on the hadron spectrum is also included.

==> plots/newcommand.tex <==

\newcommand{\warning}[1]{{\color{red} {#1}}}

\renewcommand\floatpagefraction{1}
\renewcommand\textfraction{0}

%\definecolor{stress}{rgb}{0.1,0.1,.7}
%\definecolor{current}{rgb}{1,0.5,0}
%\newcommand{\stress}[1]{{\color{stress}{#1}}}

\newcommand{\sla}[1]%
        {\kern .25em\raise.18ex\hbox{$/$}\kern-.6em #1}% Feynman slash
        

\newcommand{\gsquare}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.3]{./pics/square.pdf}}}        
\newcommand{\gcircle}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.3]{./pics/circle.pdf}}}        
\newcommand{\gphoton}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.3]{./pics/photon.pdf}}}
\newcommand{\gdllcirc}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2ll_circ.pdf}}}

\newcommand{\gocirclea}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.3]{./pics/g1circle0.pdf}}}
\newcommand{\gocircleb}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.3]{./pics/g1circle1.pdf}}}
\newcommand{\gosquarea}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.3]{./pics/g1square0.pdf}}}
\newcommand{\gosquareb}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.3]{./pics/g1square1.pdf}}}


        
\newcommand{\gou}{\raisebox{-0.0\totalheight}{\includegraphics[scale=.3]{./pics/g1u.pdf}}}
\newcommand{\god}{\raisebox{-0.0\totalheight}{\includegraphics[scale=.3]{./pics/g1d.pdf}}}
\newcommand{\gol}{\raisebox{-0.0\totalheight}{\includegraphics[scale=.3]{./pics/g1l.pdf}}}
\newcommand{\goi}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.3]{./pics/g1i.pdf}}}
\newcommand{\goip}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.3]{./pics/g1ip.pdf}}}

\newcommand{\golvert}{\raisebox{-0.0\totalheight}{\includegraphics[scale=.3]{./pics/g1l_vert.pdf}}}
\newcommand{\golself}{\raisebox{-0.15\totalheight}{\includegraphics[scale=.3]{./pics/g1l_self.pdf}}}
\newcommand{\goidisc}{\raisebox{-0.0\totalheight}{\includegraphics[scale=.3]{./pics/g1i_disc.pdf}}}
\newcommand{\goipdisc}{\raisebox{-0.0\totalheight}{\includegraphics[scale=.3]{./pics/g1ip_disc.pdf}}}
\newcommand{\goiplaq}{\raisebox{-0.0\totalheight}{\includegraphics[scale=.3]{./pics/g1i_plaq.pdf}}}
\newcommand{\goitplaq}{\raisebox{-0.0\totalheight}{\includegraphics[scale=.3]{./pics/g1i_tplaq.pdf}}}
\newcommand{\goltad}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.3]{./pics/g1l_tad.pdf}}}
\newcommand{\golltad}{\raisebox{-0.0\totalheight}{\includegraphics[scale=.3]{./pics/g1l_ltad.pdf}}}
\newcommand{\golvp}{\raisebox{-0.0\totalheight}{\includegraphics[scale=.3]{./pics/g1l_vp1.pdf}}}
\newcommand{\golvpp}{\raisebox{-0.0\totalheight}{\includegraphics[scale=.3]{./pics/g1l_vp2.pdf}}}
\newcommand{\golvppp}{\raisebox{-0.0\totalheight}{\includegraphics[scale=.3]{./pics/g1l_vp3.pdf}}}

\newcommand{\plaq}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.35]{./pics/plaq.pdf}}}
\newcommand{\vpz}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.3]{./pics/vp0.pdf}}}
\newcommand{\vp}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.3]{./pics/vp1.pdf}}}
\newcommand{\vpp}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.3]{./pics/vp2.pdf}}}
\newcommand{\vppp}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.3]{./pics/vp3.pdf}}}

        
\newcommand{\gdud}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2ud.pdf}}}
\newcommand{\gdil}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2il.pdf}}}
\newcommand{\gdll}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2ll.pdf}}}
\newcommand{\gdsi}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2si.pdf}}}
\newcommand{\gdsip}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2sip.pdf}}}
\newcommand{\gdsil}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2sil.pdf}}}
\newcommand{\gdsipl}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2sipl.pdf}}}
\newcommand{\gdnsi}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2nsi.pdf}}}
\newcommand{\gdsu}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2su.pdf}}}
\newcommand{\gduu}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2uu.pdf}}}
\newcommand{\gddd}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2dd.pdf}}}
\newcommand{\gdli}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2li.pdf}}}
\newcommand{\gdlip}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2li5.pdf}}}
\newcommand{\gdsd}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2sd.pdf}}}
\newcommand{\gdsl}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2sl.pdf}}}

\newcommand{\gdslselfs}{\raisebox{-0.22\totalheight}{\includegraphics[scale=.18]{./pics/g2sl_selfs.pdf}}}
\newcommand{\gdslselfl}{\raisebox{-0.6\totalheight}{\includegraphics[scale=.18]{./pics/g2sl_selfl.pdf}}}
\newcommand{\gdslexch}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2sl_exch.pdf}}}

\newcommand{\gdllself}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2ll_self.pdf}}}
\newcommand{\gdllexch}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2ll_exch.pdf}}}
\newcommand{\discgdllexch}{\raisebox{-0.2\totalheight}{\includegraphics[scale=.3]{./pics/discg2ll_exch.pdf}}}
\newcommand{\gdlltad}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2ll_tad.pdf}}}
\newcommand{\gdlltads}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2ll_tads.pdf}}}
\newcommand{\gdlltadf}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2ll_tadf.pdf}}}
\newcommand{\gdllphtad}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g2ll_phtad.pdf}}}

\newcommand{\gvdll}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/gv2ll.pdf}}}
\newcommand{\gvdlip}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/gv2li5.pdf}}}
\newcommand{\gvdllself}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/gv2ll_self.pdf}}}
\newcommand{\gvdllexch}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/gv2ll_exch.pdf}}}
\newcommand{\gvdllphtad}{\raisebox{-0.25\totalheight}{\includegraphics[scale=.18]{./pics/gv2ll_phtad.pdf}}}


\newcommand{\gdsltad}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2sl_tadl.pdf}}}
\newcommand{\gdsltads}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2sl_tads.pdf}}}
\newcommand{\gdsltadf}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2sl_tadf.pdf}}}

\newcommand{\gdslltad}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2sl_ltadl.pdf}}}
\newcommand{\gdslltads}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2sl_ltads.pdf}}}
\newcommand{\gdslltadf}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2sl_ltadf.pdf}}}
\newcommand{\gdslphtads}{\raisebox{-0.2\totalheight}{\includegraphics[scale=.18]{./pics/g2sl_phtads.pdf}}}
\newcommand{\gdslphtadl}{\raisebox{-0.6\totalheight}{\includegraphics[scale=.18]{./pics/g2sl_phtadl.pdf}}}

\newcommand{\gdii}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/g2ii.pdf}}}
\newcommand{\discgdii}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.3]{./pics/discg2ii.pdf}}}

\newcommand{\notdiscgdllexch}{\raisebox{-0.2\totalheight}{\includegraphics[scale=.22]{pics/notdiscg2ll_exch.pdf}}}

\newcommand{\notgdslltadf}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{pics/notg2sl_ltadf.pdf}}}

\newcommand{\protond}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.16]{./pics/uud_1.pdf}}}
\newcommand{\neutrond}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.16]{./pics/udd_1.pdf}}}
\newcommand{\protondlll}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.16]{./pics/lll_1.pdf}}}
\newcommand{\protondill}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.16]{./pics/ill_1.pdf}}}
\newcommand{\protondlil}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.16]{./pics/lil_1.pdf}}}
\newcommand{\protondlli}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.16]{./pics/lli_1.pdf}}}


\newcommand{\protonc}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.16]{./pics/uud_2.pdf}}}
\newcommand{\neutronc}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.16]{./pics/udd_2.pdf}}}
\newcommand{\protonclll}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.16]{./pics/lll_2.pdf}}}
\newcommand{\protoncill}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.16]{./pics/ill_2.pdf}}}
\newcommand{\protonclil}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.16]{./pics/lil_2.pdf}}}
\newcommand{\protonclli}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.16]{./pics/lli_2.pdf}}}
        
        
        
        
\newcommand{\discgtsud}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/discg3sud.pdf}}}        
\newcommand{\discgtsuu}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/discg3suu.pdf}}}        
\newcommand{\discgtsll}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/discg3sll.pdf}}}        
\newcommand{\discgtsil}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/discg3sil.pdf}}}        
\newcommand{\discgtils}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/discg3ils.pdf}}}        
\newcommand{\discgtsli}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/discg3sli.pdf}}}        
\newcommand{\ins}{\raisebox{-0.4\totalheight}{\includegraphics[scale=.18]{./pics/ins.pdf}}}



\newcommand{\gtsli}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3sli.pdf}}}
\newcommand{\gtils}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3ils.pdf}}}

\newcommand{\gtcus}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3cus.pdf}}}
\newcommand{\gtcds}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3cds.pdf}}}
\newcommand{\gtcls}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3cls.pdf}}}
\newcommand{\gtcis}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3cis.pdf}}}

\newcommand{\gtsuc}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3suc.pdf}}}
\newcommand{\gtsdc}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3sdc.pdf}}}
\newcommand{\gtslc}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3slc.pdf}}}
\newcommand{\gtsic}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3sic.pdf}}}

\newcommand{\gtcuc}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3cuc.pdf}}}
\newcommand{\gtcdc}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3cdc.pdf}}}
\newcommand{\gtclc}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3clc.pdf}}}
\newcommand{\gtcic}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3cic.pdf}}}


\newcommand{\gtsuu}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3suu.pdf}}}
\newcommand{\gtsil}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3sil.pdf}}}
\newcommand{\gtlis}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3lis.pdf}}}
\newcommand{\gtsll}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3sll.pdf}}}
\newcommand{\gtlls}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3lls.pdf}}}
\newcommand{\gtudu}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3udu.pdf}}}
\newcommand{\gtill}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3ill.pdf}}}
\newcommand{\gtlli}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3lli.pdf}}}
\newcommand{\gtlil}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3lil.pdf}}}
\newcommand{\gtlll}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3lll.pdf}}}
\newcommand{\gtnlll}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.2]{./pics/g3lll.pdf}}}
\newcommand{\gtnsls}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.2]{./pics/g3sls.pdf}}}
\newcommand{\gtsdu}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3sdu.pdf}}}
\newcommand{\gtsls}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3sls.pdf}}}
\newcommand{\gtsis}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3sis.pdf}}}
\newcommand{\gtsus}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3sus.pdf}}}
\newcommand{\gtsds}{\raisebox{-0.3\totalheight}{\includegraphics[scale=.18]{./pics/g3sds.pdf}}}

%\newcommand{\be}{\begin{displaymath}}
%\newcommand{\ee}{ \end{displaymath}}
%\newcommand{\ben}{\begin{equation}}
%\newcommand{\een}{ \end{equation}}
%\newcommand{\be}{\begin{equation}}
%\newcommand{\ee}{ \end{equation}}
%\newcommand{\bea}{\begin{eqnarray*}}
%\newcommand{\eea}{ \end{eqnarray*}}
%\newcommand{\bea}{\begin{eqnarray}}
%\newcommand{\eea}{ \end{eqnarray}}
%\newcommand{\bear}[1]{\begin{displaymath}\begin{array}{#1}}
%\newcommand{\eear}{ \end{array}\end{displaymath}}
\newcommand{\bear}[1]{\begin{equation}\begin{array}{#1}}
\newcommand{\eear}{ \end{array}\end{equation}}
\newcommand{\barr}[1]{\begin{array}{#1}}
\newcommand{\earr}{\end{array}}
 
\newcommand{\half}{\ensuremath{\frac{1}{2} }}

\newcommand{\ket}[1]{\ensuremath{| {#1} \rangle }}
\newcommand{\bra}[1]{\ensuremath{\langle {#1} |}}
\newcommand{\braOket}[3]{\ensuremath{\bra{#1}{#2}\ket{#3} }}
\newcommand{\braket}[2]{\ensuremath{\langle {#1} | {#2} \rangle}}
\newcommand{\averO}[1]{\ensuremath{\langle {#1}\rangle }}
	
%%
%% form factors
%%
\newcommand {\fp}{\ensuremath{f_+ (q^2)}}
\newcommand {\fm}{\ensuremath{f_- (q^2)}}


